Probing the flavour-blind SMEFT: EFT validity and the interplay of energy scales

The Standard Model Effective Field Theory (SMEFT) offers a systematic approach to study potential deviations from the Standard Model (SM) through higher-dimensional operators that encapsulate new physics effects. In this work, we analyze flavour-blind SMEFT contributions to flavour observables and assess their interplay with high-energy measurements from LEP and LHC. We perform global fits combining LEP precision data, flavour observables from rare B-meson decays, and LHC diboson measurements, revealing how the inclusion of different datasets breaks parameter degeneracies and enhances the sensitivity to SMEFT coefficients. Our study demonstrates that low-energy flavour observables provide reliable constraints even in flavour-blind scenarios, while high-energy measurements can be subject to EFT validity concerns due to kinematic growth. We investigate the impact of renormalization group evolution (RGE) and operator mixing across energy scales, highlighting the complementary nature of low- and high-energy datasets. The results emphasize the importance of flavour observables as robust probes of new physics and underline the necessity of global fits to avoid potential biases from limited datasets. Finally, we discuss the implications of our findings for the interpretation of global SMEFT analyses based on high-energy collider data, comparing UV models that contribute to SMEFT at tree- and loop-level.

==> sec-flavour-obs.tex <==
\Luca{This is the OLD section of flavour observables}
\section{Flavour observables and flavour-blind SMEFT contributions}
\label{sec:flavour_observables}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/TGCs.png}
    \caption{From Ref~\cite{Bobeth:2015zqa}}
    %\label{fig:enter-label}
\end{figure}
In this section we discuss how flavour observables provide a powerful testing ground for SMEFT, as they are sensitive to new physics effects at both low and high energies. Flavour-blind SMEFT operators, which assume no explicit breaking of the Standard Model's flavour symmetries, can influence flavour observables in subtle but measurable ways. These effects often manifest in rare decays, mixing phenomena, and CP violation, where precision measurements impose stringent constraints.

Recent work has explored the interplay between flavour-blind SMEFT contributions and flavour observables. A notable example is the pair of studies~\cite{Greljo:2023adz, Greljo:2023bdy}, which examine flavour-blind scenarios using flavour observables to constrain new physics. Additionally, other works by Greljo and collaborators~\cite{Greljo:2023bab, Greljo:2022cah, Greljo:2022jac} explore the impact of flavour observables and their interplay with high-energy data, providing insights into how SMEFT effects propagate across energy scales.

Global fits have also been instrumental in investigating the relationship between flavour and high-energy observables~\cite{Bartocci:2023nvp, Bruggisser:2022rhb, Aoude:2020dwv, Bruggisser:2021duo}. These studies consider different flavour scenarios, with a primary focus on Minimal Flavour Violation (MFV). Such fits highlight the potential of combining flavour and collider data to constrain SMEFT parameter spaces.

Finally, the work in~\cite{Hurth:2019ula} is particularly relevant for understanding the matching between SMEFT and the Weak Effective Theory (WET), a critical step for accurately translating high-energy constraints to low-energy flavour observables. This calculation serves as a bridge between SMEFT operators and the observables measured in experiments, enabling robust tests of flavour-blind SMEFT scenarios.

We now move onto discussing the translation between the anomalous TGC Lagrangian in Eq.~\ref{eq:WWW} and low energy observables at the $b$ scale. 

In particular, if we consider the WET Lagrangian:

\begin{equation}
    \mathcal{L}_{|\Delta B|=|\Delta S|=1}=\frac{4 G_F}{\sqrt{2}} V_{t s}^* V_{t b}\left(C_7 \OO_7+C_9 \OO_9+C_{10} \OO_{10}\right)+\text { h.c. } \, ,
\end{equation}
where the Wilson coefficients are $C_i = C_i^{SM} + \Delta C_i$ and the WET operators are given by
\begin{align}
\OO_7 & =\frac{e}{(4 \pi)^2} m_b\left(\bar{s}_L \sigma_{\alpha \beta} b_R\right) F^{\alpha \beta} \\
\OO_9 & =\frac{e^2}{(4 \pi)^2}\left(\bar{s}_L \gamma_\alpha b_L\right)\left(\bar{\ell} \gamma^\alpha \ell\right) \\
\OO_{10} & =\frac{e^2}{(4 \pi)^2}\left(\bar{s}_L \gamma_\alpha b_L\right)\left(\bar{\ell} \gamma^\alpha \gamma_5 \ell\right) \, .
\end{align}

The matching from the TGC to the WET Lagrangian yields
\begin{align}
\Delta C_7 & =\Delta \kappa_\gamma f_7^\kappa\left(x_t\right)+\lambda_\gamma f_7^\lambda\left(x_t\right) \\
\Delta C_9 & =-\Delta D+\lambda_\gamma f_9^\lambda\left(x_t\right)+\frac{1-4 s_w^2}{s_w^2} \Delta C \\
\Delta C_{10} & =-\frac{1}{s_w^2} \Delta C \ ,
\end{align}
with $x_t = m_t^2/m_W^2$ and
\begin{align}
f_7^\kappa(x) &=-\frac{x}{2(x-1)^2}-\frac{x^3-3 x^2}{4(x-1)^3} \ln x \\
f_7^\lambda(x) &=\frac{x^2+x}{4(x-1)^2}-\frac{x^2}{2(x-1)^3} \ln x \\
f_9^\lambda(x) &=-\frac{3 x^2-x}{2(x-1)^2}+\frac{x^3}{(x-1)^3} \ln x \ ,
\end{align}
and the Z and $\gamma$ penguin diagrams are encoded in
\begin{equation}
    \Delta C=\frac{3 c_w^2}{8} \Delta g_1^Z x_t \ln \left(\frac{\Lambda^2}{m_W^2}\right), \quad \Delta D=\frac{1}{4} \Delta \kappa_\gamma x_t \ln \left(\frac{\Lambda^2}{m_W^2}\right) .
\end{equation}
In addition to these, also the coupling of the Z boson to the $b$ quarks is affected, i.e.
\begin{equation}
    \mathcal{L}_{Z b \bar{b}}=\frac{e}{s_w c_w}\left[\left(g_L^b+\delta g_L^b\right) \bar{b}_L \not b_L+g_R^b \bar{b}_R \not b_R\right] ,
\end{equation}
and the induced anomalous coupling is given by
\begin{align}
\delta g_L^b &=\frac{\alpha}{2 \pi s_w^2}\left|V_{t b}\right|^2(\Delta C+\delta C) \, , \\
\delta C &=\frac{1}{16} \Delta \kappa_Z x_t \ln \left(\frac{\Lambda^2}{m_W^2}\right) \, .
\end{align}

{\bf NOTE: only LL is included in the calculations.}


\subsection{Flavour Observables}
\label{sec:flavourobs}

{\bf Place this in an appendix?}

By comparing measured branching ratios, CP asymmetries, and other flavour-sensitive quantities to their SM predictions, we can infer constraints on potential SMEFT contributions, particularly those from flavour-blind operators. 

In this section, we present a summary of the relevant flavour observables, their experimental measurements, and their Standard Model predictions. Additionally, we calculate the ratios of experimental measurements to SM predictions to quantify any deviations. 

Table~\ref{tab:observables} lists the flavour observables considered in this study, along with their theoretical expressions within the SMEFT framework. The observables are parameterized in terms of SMEFT Wilson coefficients, such as $\Delta C_7$, $\Delta C_{10}$, and $\Delta C$, which encapsulate the effects of new physics.


\begin{table}[h!]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Observable} & \textbf{Expression} \\ \hline
$R_{X_s}$ & $\frac{\operatorname{Br}\left(B \rightarrow X_s \gamma\right)}{\operatorname{Br}\left(B \rightarrow X_s \gamma\right)_{\mathrm{SM}}}=1-2.45 \Delta C_7 $ \\ \hline
$R_{\mu^{+} \mu^{-}}$ & $\frac{\operatorname{Br}\left(B_s \rightarrow \mu^{+} \mu^{-}\right)}{\operatorname{Br}\left(B_s \rightarrow \mu^{+} \mu^{-}\right)_{\mathrm{SM}}}=\left(1-0.25 \Delta C_{10}\right)^2$ \\ \hline
$\delta g_L^b$ & - \\ \hline
$R_{K^+}$ & $\frac{\operatorname{Br}\left(K^+ \rightarrow \pi^+ \nu \bar{\nu}\right)}{\operatorname{Br}\left(K^+ \rightarrow \pi^+ \nu \bar{\nu}\right)_{\mathrm{SM}}} = 1 + 0.93 \Delta C + 0.22 (\Delta C)^2$ \\ \hline
$R_{K^0}$ & $\frac{\operatorname{Br}\left(K^0_L \rightarrow \pi^0 \nu \bar{\nu}\right)}{\operatorname{Br}\left(K^0_L \rightarrow \pi^0 \nu \bar{\nu}\right)_{\mathrm{SM}}} = 1 + 1.36 \Delta C + 0.46 (\Delta C)^2$ \\ \hline
$\epsilon^{\prime}/{\epsilon}$ & $\left(-2.3+21.0 R_6-8.0 R_8+\left[\left(1.2+0.2 R_6\right) \Delta C+\left(0.9-16.2 R_8\right) \Delta Z\right]\right) \cdot 10^{-4}$ \\ \hline
\end{tabular}
\caption{Flavour observables and their expressions in terms of SMEFT parameters.}
\label{tab:observables}
\end{table}

In the above, $R_8$ can be extracted from~\cite{Blum:2015ywa} as $R_8 = 6.6/8.0 = 0.83$. With the SM prediction quoted below, we can then extract $R_6=1.092$ to be consistent with it.


Table~\ref{tab:measurements} summarizes the latest experimental results for the relevant observables, including measurements of $B \rightarrow X_s \gamma$, $B_s \rightarrow \mu^+ \mu^-$, $K^+ \rightarrow \pi^+ \nu \bar{\nu}$, $K^0_L \rightarrow \pi^0 \nu \bar{\nu}$, and $\epsilon^\prime / \epsilon$. These results are derived from high-precision experiments, with uncertainties reflecting the current state of experimental knowledge.


\begin{table}[h!]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Observable} & \textbf{Measurement} \\ \hline
$\operatorname{Br}\left(B \rightarrow X_s \gamma\right)$ & $(3.49 \pm 0.19) \cdot 10^{-4}$ \href{https://pdglive.lbl.gov/BranchingRatio.action?desig=225&parCode=S049&expand=true}{PDG-link} \\ \hline
$\operatorname{Br}\left(B_s \rightarrow \mu^{+} \mu^{-}\right)$ & $(3.34 \pm 0.27) \cdot 10^{-9}$ \href{https://pdglive.lbl.gov/BranchingRatio.action?pdgid=S086.15&home=MXXX046}{PDG-link} \\ \hline
$\operatorname{Br}\left(K^+ \rightarrow \pi^+ \nu \bar{\nu}\right)$ & $(10.9 \pm 4.6) \cdot 10^{-11}$ \cite{NA62:2021zjw} \\ \hline
$\operatorname{Br}\left(K^0_L \rightarrow \pi^0 \nu \bar{\nu}\right)$ & $\le 8.14 \cdot 10^{-10}$ \cite{annurev:/content/journals/10.1146/annurev-nucl-102419-054905, Grossman:1997sk} \\ \hline
$\epsilon^\prime / \epsilon$ & $(16.6 \pm 2.3)\cdot 10^{-4}$ \href{https://pdglive.lbl.gov/ParticleGroup.action?init=0&node=MXXX020}{PDG-link} \\ \hline
\end{tabular}
\caption{Experimental measurements of flavour observables.}
\label{tab:measurements}
\end{table}



Table~\ref{tab:sm_predictions} provides the corresponding Standard Model predictions for the same set of observables. These predictions are obtained from detailed theoretical calculations, incorporating higher-order corrections and the latest input parameters. They serve as benchmarks for identifying potential deviations arising from new physics.


\begin{table}[h!]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Observable} & \textbf{SM Prediction} \\ \hline
$\operatorname{Br}\left(B \rightarrow X_s \gamma\right)$ & $(3.40 \pm 0.17) \cdot 10^{-4}$ \cite{Misiak_2020, Czaja:2023ren} \\ \hline
$\operatorname{Br}\left(B_s \rightarrow \mu^{+} \mu^{-}\right)$ & $(3.64 \pm 0.12) \cdot 10^{-9}$ \cite{Czaja:2024the} \\ \hline
$\operatorname{Br}\left(K^+ \rightarrow \pi^+ \nu \bar{\nu}\right)$ & $(8.1 \pm 0.4) \cdot 10^{-11}$ \href{https://pdglive.lbl.gov/ParticleGroup.action?init=0&node=MXXX020}{PDG-link} \\ \hline
$\operatorname{Br}\left(K^0_L \rightarrow \pi^0 \nu \bar{\nu}\right)$ & $(2.8 \pm 0.2) \cdot 10^{-11}$ \href{https://pdglive.lbl.gov/ParticleGroup.action?init=0&node=MXXX020}{PDG-link} \\ \hline
$\epsilon^\prime / \epsilon$ & $(14 \pm 5)\cdot 10^{-4}$ \cite{Cirigliano:2019cpi} \\ \hline
\end{tabular}
\caption{Standard Model predictions for flavour observables.}
\label{tab:sm_predictions}
\end{table}



Finally, Table~\ref{tab:ratios} presents the ratios of the experimental measurements to the Standard Model predictions for each observable. These ratios highlight any potential deviations, with values close to unity indicating consistency with the SM. Significant deviations could signal the presence of new physics, motivating further study and constraints on SMEFT Wilson coefficients.




\begin{table}[h!]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Ratio} & \textbf{Value} \\ \hline
$R_{X_s}$ & $1.026 \pm 0.076$ \\ \hline
$R_{\mu^{+} \mu^{-}}$ & $0.918 \pm 0.080$ \\ \hline
$R_{K^{+}}$ & $1.35 \pm 0.6$ \\ \hline
$R_{K^0}$ & $\le 29.1$ \\ \hline
\end{tabular}
\caption{Ratios of measured values to Standard Model predictions.}
\label{tab:ratios}
\end{table}

==> test_feynman_diagram.tex <==
\begin{tikzpicture}
  \begin{feynman}
    \vertex (i1) at (-2, 0) {$Z$};
    \node[dot, black] (v1) at (-0.5, 0);
    \node[dot, black] (v2) at (0.5, 0.5);
    \node[dot, black] (v3) at (0.5, -0.5);
    \vertex (f1) at (1.5, 1);
    \vertex (f2) at (1.5, -1);
    \vertex (f3) at (2.5, 1.5) {$l^+$};
    \vertex (f4) at (2.5, 0.5) {$l^-$};
    \vertex (f5) at (2.5, -1.5) {$l$};
    \vertex (f6) at (2.5, -0.5) {$\nu$};
    \diagram* {
    (i1) -- [photon, line width=0.3mm] (v1) -- [line width=0.5mm] (v2) -- [photon, line width=0.3mm, , edge label=$W^+$] (f1),
    (v3) -- [photon, line width=0.3mm, edge label=$W^-$] (f2),
    (v2) -- [line width=0.5mm] (v3) -- [line width=0.5mm] (v1),
    (f4) -- [fermion, line width=0.3mm] (f1) -- [fermion, line width=0.3mm] (f3),
    (f5) -- [fermion, line width=0.3mm] (f2) -- [fermion, line width=0.3mm] (f6),
    };
  \end{feynman}
\end{tikzpicture}

